CondenseNet: An Efficient DenseNet using Learned Group Convolutions

Deep neural networks are increasingly used on mobile devices, where computational resources are limited. In this paper we develop CondenseNet, a novel network architecture with unprecedented efficiency. It combines dense connectivity with a novel module called learned group convolution. The dense connectivity facilitates feature re-use in the network, whereas learned group convolutions remove connections between layers for which this feature re-use is superfluous. At test time, our model can be implemented using standard group convolutions, allowing for efficient computation in practice. Our experiments show that CondenseNets are far more efficient than state-of-the-art compact convolutional networks such as MobileNets and ShuffleNets.

==> abstractSicher.tex <==
%!TEX root = main.tex
Deep neural networks are increasingly used on mobile devices with severe hardware limitations. Although mobile devices have stringent hardware restrictions, the models are typically still trained on standard GPU servers. In this paper we propose a novel  convolutional network architecture which allows for maximum

Ideally these specialized architectures should still take advantage of GPU support during training,  to facilitate rapid development cycles and model selection. 
In this paper, we develop a novel convolutional network architecture, which we refer to as \condense{}, that combines dense connectivity between layers at different levels with a mechanism to remove unused connections. The dense connectivity facilitates feature re-use where necessary, but we remove connections between layers for which feature re-use is superfluous. At test time, our model can be implemented using standard grouped convolutions, allowing for efficient computation in practice. Our experiments demonstrate that \condense{}s are significantly more efficient than previous state-of-the-art compact convolutional networks, such as MobileNets and ShuffleNets.

%Designing compact convolutional networks is essential for real-world applications on limited computational resources, e.g., self-driving cars or mobile devices. In this paper, we develop a novel convolutional network architecture, which we refer to as \condense{}, that combines dense connectivity between layers at different levels with a mechanism to remove unused connections. The dense connectivity facilitates feature re-use where necessary, but we remove connections between layers for which feature re-use is superfluous. At test time, our model can be implemented using standard grouped convolutions, allowing for efficient computation in practice. Our experiments demonstrate that \condense{}s are significantly more efficient than previous state-of-the-art compact convolutional networks, such as MobileNets and ShuffleNets.

 %the highly efficient DenseNet architecture, and introduce a specially designed algorithm to further enhance its computational efficiency. The algorithm is able to automatically screen out redundant connections during the course of training, yielding a sparse connectivity pattern. However, the obtained model is still ``dense" in two aspects that make it even more appealing: (1) the sparsified convolutional layers can be cast into standard grouped convolution, which allows efficient dense matrix operations; (2) there still exist dense connections across layers, enabling effective feature reuse. To further exploit the power of this algorithm, we also introduce an improved DenseNet architecture which enables a more extensive feature reuse in the network. We empirically show that our obtained model, named \condense, significantly outperforms the original DenseNets and the recently proposed efficient models for mobile applications, e.g., MobileNets and ShuffleNets, in terms of computational efficiency.


%we first present a variant of DenseNets, named \modelname, which has direct dense connections between any two convolutional layers, even their produced feature maps have different resolutions. Such full dense connectivity enables an extensive feature reuse in the network, and leads to significantly improved computational efficiency. Then we introduce a method to automatically screen out redundant connections during the course of training. This forces the network to selectively reusing most significant features from the feature pool, yielding a even more condensed model. We call the method {\methodname}, as a structured sparsity is enforced on the convolutional layers so they can be casted as {grouped convolution} afterwards, while the groups is formed during the learning process, instead of being predefined. We empirically show that the condensed networks with \methodname{} significantly outperform the recently proposed efficient models for mobile applications, e.g., MobileNets and ShuffleNets, in terms of computational efficiency.




==> arXiv 20180607/abstract.tex <==
%!TEX root=main.tex
Deep neural networks are increasingly used on mobile devices, where computational resources are limited. In this paper we develop \condense{}, a novel network architecture with unprecedented efficiency.
It combines dense connectivity with a novel module called \methodname{}. The dense connectivity facilitates feature re-use in the network, whereas \methodname{}s remove connections between layers for which this feature re-use is superfluous. At test time, our model can be implemented using standard group convolutions, allowing for efficient computation in practice. Our experiments show that \condense{}s are far more efficient than state-of-the-art compact convolutional networks such as ShuffleNets.

% Typically the models are typically still trained on standard GPU servers. In this paper we propose a novel  convolutional network architecture which allows for maximum

% Ideally these specialized architectures should still take advantage of GPU support during training,  to facilitate rapid development cycles and model selection.
% In this paper, we develop a novel convolutional network architecture, which we refer to as \condense{}, that combines dense connectivity between layers at different levels with a mechanism to remove unused connections. The dense connectivity facilitates feature re-use where necessary, but we remove connections between layers for which feature re-use is superfluous. At test time, our model can be implemented using standard grouped convolutions, allowing for efficient computation in practice. Our experiments demonstrate that \condense{}s are significantly more efficient than previous state-of-the-art compact convolutional networks, such as MobileNets and ShuffleNets.


%Designing compact convolutional networks is essential for real-world applications in which computational resources are limited, e.g., self-driving cars or mobile devices. In this paper, we develop a novel network architecture, called \condense{}, that combines dense connectivity between layers with a mechanism to remove unused connections, called \methodname{}. The dense connectivity facilitates feature re-use in the network, whereas \methodname{}s remove connections between layers for which this feature re-use is superfluous. At test time, our model can be implemented using standard grouped convolutions, allowing for efficient computation in practice. Our experiments demonstrate that \condense{}s are much more efficient than state-of-the-art compact convolutional networks such as MobileNets and ShuffleNets.

 %the highly efficient DenseNet architecture, and introduce a specially designed algorithm to further enhance its computational efficiency. The algorithm is able to automatically screen out redundant connections during the course of training, yielding a sparse connectivity pattern. However, the obtained model is still ``dense" in two aspects that make it even more appealing: (1) the sparsified convolutional layers can be cast into standard grouped convolution, which allows efficient dense matrix operations; (2) there still exist dense connections across layers, enabling effective feature reuse. To further exploit the power of this algorithm, we also introduce an improved DenseNet architecture which enables a more extensive feature reuse in the network. We empirically show that our obtained model, named \condense, significantly outperforms the original DenseNets and the recently proposed efficient models for mobile applications, e.g., MobileNets and ShuffleNets, in terms of computational efficiency.


%we first present a variant of DenseNets, named \modelname, which has direct dense connections between any two convolutional layers, even their produced feature maps have different resolutions. Such full dense connectivity enables an extensive feature reuse in the network, and leads to significantly improved computational efficiency. Then we introduce a method to automatically screen out redundant connections during the course of training. This forces the network to selectively reusing most significant features from the feature pool, yielding a even more condensed model. We call the method {\methodname}, as a structured sparsity is enforced on the convolutional layers so they can be casted as {grouped convolution} afterwards, while the groups is formed during the learning process, instead of being predefined. We empirically show that the condensed networks with \methodname{} significantly outperform the recently proposed efficient models for mobile applications, e.g., MobileNets and ShuffleNets, in terms of computational efficiency.




==> arXiv 20180607/abstractSicher.tex <==
%!TEX root = main.tex
Deep neural networks are increasingly used on mobile devices with severe hardware limitations. Although mobile devices have stringent hardware restrictions, the models are typically still trained on standard GPU servers. In this paper we propose a novel  convolutional network architecture which allows for maximum

Ideally these specialized architectures should still take advantage of GPU support during training,  to facilitate rapid development cycles and model selection. 
In this paper, we develop a novel convolutional network architecture, which we refer to as \condense{}, that combines dense connectivity between layers at different levels with a mechanism to remove unused connections. The dense connectivity facilitates feature re-use where necessary, but we remove connections between layers for which feature re-use is superfluous. At test time, our model can be implemented using standard grouped convolutions, allowing for efficient computation in practice. Our experiments demonstrate that \condense{}s are significantly more efficient than previous state-of-the-art compact convolutional networks, such as MobileNets and ShuffleNets.

%Designing compact convolutional networks is essential for real-world applications on limited computational resources, e.g., self-driving cars or mobile devices. In this paper, we develop a novel convolutional network architecture, which we refer to as \condense{}, that combines dense connectivity between layers at different levels with a mechanism to remove unused connections. The dense connectivity facilitates feature re-use where necessary, but we remove connections between layers for which feature re-use is superfluous. At test time, our model can be implemented using standard grouped convolutions, allowing for efficient computation in practice. Our experiments demonstrate that \condense{}s are significantly more efficient than previous state-of-the-art compact convolutional networks, such as MobileNets and ShuffleNets.

 %the highly efficient DenseNet architecture, and introduce a specially designed algorithm to further enhance its computational efficiency. The algorithm is able to automatically screen out redundant connections during the course of training, yielding a sparse connectivity pattern. However, the obtained model is still ``dense" in two aspects that make it even more appealing: (1) the sparsified convolutional layers can be cast into standard grouped convolution, which allows efficient dense matrix operations; (2) there still exist dense connections across layers, enabling effective feature reuse. To further exploit the power of this algorithm, we also introduce an improved DenseNet architecture which enables a more extensive feature reuse in the network. We empirically show that our obtained model, named \condense, significantly outperforms the original DenseNets and the recently proposed efficient models for mobile applications, e.g., MobileNets and ShuffleNets, in terms of computational efficiency.


%we first present a variant of DenseNets, named \modelname, which has direct dense connections between any two convolutional layers, even their produced feature maps have different resolutions. Such full dense connectivity enables an extensive feature reuse in the network, and leads to significantly improved computational efficiency. Then we introduce a method to automatically screen out redundant connections during the course of training. This forces the network to selectively reusing most significant features from the feature pool, yielding a even more condensed model. We call the method {\methodname}, as a structured sparsity is enforced on the convolutional layers so they can be casted as {grouped convolution} afterwards, while the groups is formed during the learning process, instead of being predefined. We empirically show that the condensed networks with \methodname{} significantly outperform the recently proposed efficient models for mobile applications, e.g., MobileNets and ShuffleNets, in terms of computational efficiency.




==> arXiv 20180607/background.tex <==
%!TEX root = main.tex

\begin{figure*}[t]
  % Requires \usepackage{graphicx}
  \centering
  \includegraphics[width=1.0 \textwidth]{plots/learned_conv.pdf}\\
%  \hspace{0.01 \textwidth}
  \caption{Illustration of \methodname{}s with $G \!=\! 3$ groups and a condensation factor of $C \!=\! 3$. During training a fraction of $(C\!-\!1)/C$ connections are removed after each of the $C-1$ condensing stages. Filters from the same group use the same set of features, and during test-time the \emph{index layer} rearranges the features to allow the  resulting model to be implemented as standard group convolutions.}\label{fig:learned_conv}
  \vspace{-2ex}
\end{figure*}

\vspace{-1ex}
\subsection{DenseNet}
\vspace{-1ex}
Densely connected networks (DenseNets; \cite{huang2017densely}) consist of multiple \emph{dense blocks}, each of which consists of multiple \emph{layers}. Each layer produces $k$ features, where $k$ is referred to as the \emph{growth rate} of the network. The distinguishing property of DenseNets is that the input of each  layer is a concatenation of all feature maps generated by \emph{all} preceding layers within the same dense block. 
%The $\ell^{th}$ layer therefore receives $\ell k$ input channels.
Each  layer performs a sequence of consecutive  transformations, as shown in the left part of \figurename~\ref{fig:structure_compare}.  The first transformation (\emph{BN-ReLU}, blue) is a composition of {batch normalization} \cite{batch-norm} and {rectified linear units} \cite{nair2010rectified}.
The first convolutional layer in the sequence reduces the number of channels to save computational cost by using the $1\!\times\! 1$ filters. The output is followed by another BN-ReLU transformation and is then reduced to the final $k$ output features through a $3\!\times \!3$ convolution.
% A \emph{transition layer} is used to perform down-sampling of the feature maps between two contiguous dense blocks.
% In a typical DenseNet, the number of new feature maps produced by each basic layer, , is much smaller than in other CNN architectures.
% The dense connectivity encourages feature re-use and reduces redundancy. The majority of the computational cost is incurred in the $1\times 1$ convolution

\vspace{-1ex}
\subsection{Group Convolution}
\vspace{-1ex}
\label{sec:group-conv}
Group convolution is a special case of a sparsely connected convolution, as illustrated in \figurename~\ref{fig:group-conv}. It was first used in the AlexNet architecture \cite{alexnet}, and has more recently been popularized by their successful application in ResNeXt \cite{resnext}. Standard convolutional layers (left illustration in \figurename~\ref{fig:group-conv}) generate $O$ output features by applying a convolutional filter (one per output) over \emph{all} $R$ input features, leading to a computational cost of $R\times O$. In comparison, group convolution (right illustration) reduces this computational cost by partitioning the input features into $G$ mutually exclusive groups, each producing its own outputs---reducing the computational cost by a factor $G$ to $\frac{R\times O}{G}$.

%\emph{incoming features} and  \emph{filters} are split into a predefined number of groups, and connections exist only between filter groups and their corresponding feature groups. As a result, different filter groups use disjoint sets of features as input; each feature map is used by exactly one filter group.
% \paragraph{Group-convolution DenseNets.}
% Group convolution may seem particularly promising for dense architectures, where the number of input features, $R$,  can become very large in later layers. However, although it works surprisingly well in other architectures \cite{resnext,zhang2017shufflenet,zhang2017interleaved}, preliminary experiments show that a na\"ive adaptation of group convolutions in DenseNets leads to drastic reductions in accuracy. We surmise that this is caused by the fact that feature maps in DenseNets
% have an intrinsic order, as they
% are concatenations of feature maps from prior layers. The hard assignment of these (ordered) features to disjoint groups hinders effective re-use of features in the network.
% This hypothesis is supported by experiments in which we randomly permute feature maps in each layer before performing the group convolution, which reduces the negative impact on the accuracy. However, even with the random permutation, ``group-convolution DenseNets'' are still substantially less accurate than  smaller DenseNets with equivalent computational cost.

%Our results show that grouping features by preserving their original order, i.e., low-level and high-level features are assigned to different groups separately, leads to significantly worse results compared to the original DenseNet with a similar size.



==> arXiv 20180607/conclusion.tex <==
%!TEX root = main.tex
\vspace{-1ex}
\section{Conclusion}
\vspace{-1ex}
In this paper, we introduced \condense{}: an efficient convolutional network architecture that encourages feature re-use via dense connectivity and prunes filters associated with superfluous feature re-use via \methodname{}s. To make inference efficient, the pruned network can be converted into a network with regular group convolutions, which are implemented efficiently in most deep-learning libraries. Our pruning method is simple to implement, and adds only limited computational costs to the training process. In our experiments, \condense{}s outperform recently proposed MobileNets and ShuffleNets in terms of computational efficiency at the same accuracy level. \condense{} even slightly outperforms a network architecture that was discovered by empirically trying tens of thousands of convolutional network architectures, and with a much simpler structure.


==> arXiv 20180607/experiment.tex <==
%!TEX root = main.tex
%\vspace{-1ex}
\section{Experiments}
%\vspace{-1ex}
We evaluate \condense{}s on the CIFAR-10, CIFAR-100 \cite{cifar}, and the ImageNet (ILSVRC 2012; \cite{deng2009imagenet}) image-classification datasets.
%All models are trained using the PyTorch framework.
The models and code reproducing our experiments are publicly available at
{\small{\url{https://github.com/ShichenLiu/CondenseNet}}}.
%\url{https://github.com/ShichenLiu/CondenseNet}.

\paragraph{Datasets.}
The CIFAR-10 and CIFAR-100 datasets consist of RGB images of size 32$\times$32 pixels, corresponding to 10 and 100 classes, respectively. Both datasets contain 50,000 training images and 10,000 test images.
We use a standard data-augmentation scheme \cite{netinnet, fitnet, dsn, allcnn, highway, stochastic, fractalnet}, in which the images are zero-padded with 4 pixels on each side, randomly cropped to produce 32$\times$32 images, and horizontally mirrored with probability $0.5$.

The ImageNet dataset comprises 1000 visual classes, and contains a total of 1.2 million training images and 50,000 validation images. We adopt the data-augmentation scheme of \cite{resnet} at training time, and perform a rescaling to $256 \times 256$ followed by a $224\times 224$ center crop at test time before feeding the input image into the networks.


\begin{figure}
  % Requires \usepackage{graphicx}
  \centering
  \includegraphics[width=0.48 \textwidth]{plots/flops_vs_err.pdf}\\
  \caption{Ablation study on CIFAR-10 to investigate the efficiency gains obtained by the various components of \condense{}.}
  \label{fig:param_vs_err_pp}
\vspace{-2ex}
\end{figure}

%\begin{figure}
%  % Requires \usepackage{graphicx}
%  \centering
%  \includegraphics[width=0.50 \textwidth]{plots/param_vs_err_L.pdf}\\
%  \caption{\textit{Left}: Comparison of the computational efficiency on CIFAR between DenseNet and \todo{CondenseNet}. \textit{Right}: Comparison of the parameter efficiency on CIFAR between DenseNet and \todo{CondenseNet}.}
%  \label{fig:param_vs_err_L}
%\end{figure}

\subsection{Results on CIFAR}
\vspace{-1ex}
\label{subsec:cifar}
We first perform a set of experiments on CIFAR-10 and CIFAR-100 to validate the effectiveness of \methodname{}s and the proposed \condense{} architecture.

\paragraph{Model configurations.}
Unless otherwise specified, we use the following network configurations in all experiments on the CIFAR datasets. The standard DenseNet has a constant growth rate of $k\!=\!12$ following \cite{huang2017densely}; our proposed architecture uses growth rates $k_0\!\in\!\{8,\! 16,\! 32\}$ to ensure that the growth rate is divisable by the number of groups. The \methodname{} is only applied to the first convolutional layer (with filter size $1\!\times\! 1$, see \figurename~\ref{fig:structure_compare}) of each basic layer, with a condensation factor of $C \!=\! 4$, \emph{i.e.}, 75\% of filter weights are gradually pruned during training with a step of 25\%.  The $3\!\times\! 3$ convolutional layers are replaced by standard group convolution (without applying \methodname) with four groups. Following  \cite{zhang2017shufflenet,zhang2017interleaved}, we permute the output channels of the first $1\!\times\! 1$ learned group convolutional layer, such that the features generated by each of its groups are evenly used by all the groups of the subsequent $3\times 3$ group convolutional layer .
% obtains the same number of inputs from each group of the $1\times 1$ conv. layer.
%to increase the compatibility of two subsequent group convolution layers (see \figurename~\ref{fig:structure_compare}).


\paragraph{Training details.}
We train all models with stochastic gradient descent (SGD) using similar optimization hyper-parameters as in \cite{resnet, huang2017densely}. Specifically, we adopt Nesterov momentum with a momentum weight of 0.9 without dampening, and use a weight decay of $10^{-4}$. All models are trained with mini-batch size 64 for 300 epochs, unless otherwise specified. We use a cosine shape learning rate which starts from 0.1 and gradually reduces to 0.
%Group lasso regularization was not used in the experiments on the CIFAR datasets, as it did not lead to further accuracy improvements on those two datasets.
Dropout~\cite{dropout} with a drop rate of $0.1$ was applied to train \condense{}s with $>\!3$ million parameters (shown in Table~\ref{tab:cifar}).

\paragraph{Component analysis.}
%\lvdm{This should become a full-fledged ablation study rather than a comparison with DenseNets.}
%\condense{} differs from the original DenseNet in two ways, namely, the introduction of \methodname{} and two changes to the architecture design.
\figurename~\ref{fig:param_vs_err_pp} compares the computational efficiency gains obtained by each component of CondenseNet: learned group convolution (LGR), exponentially increasing learning rate (IGR), full dense connectivity (FDC).
% of the following four models:
% (1) the original \emph{DenseNet};
% (2) the proposed \emph{\condense} (DenseNet with \methodname{});
% (3) \condense{} with the ; and
% (4) \condense{} with the exponentially increasing learning rate and full dense connectivity (\emph{\condense{}-IGR-FDC} or \emph{\condense$^\text{Full}$} for short).
Specifically, the figure plots the test error as a function of the number of FLOPs (\emph{i.e.}, multiply-addition operations).
The large gap between the two red curves with dot markers shows that \methodname{} significantly improves the efficiency of our models. Compared to DenseNets, \condense$^{light}$ only requires half the number of FLOPs to achieve comparable accuracy.
Further, we observe that the exponentially increasing growth rate, yields even further efficiency. Full dense connectivity does not boost the efficiency significantly on CIFAR-10, but there does appear to be a trend that as models getting larger, full connectivity starts to help. We opt to include this architecture change in the \condense{} model, as it does lead to substantial improvements on ImageNet (see later).


%\paragraph{\methodnamecap.}
%\figurename~\ref{fig:param_vs_err_pp} also shows how the \methodname{} further improves the model compactness for both the original DenseNets and our proposed architecture. Roughly, \condense{} only require about 50\% to 70\% the amount of compute of their counterparts to achieve a similar performance level. Remarkably, the \condense{}  leads to a $3\times$ speedup over the original DenseNet.

\paragraph{Comparison with state-of-the-art efficient CNNs.}
In Table~\ref{tab:cifar}, we show the results of experiments comparing a 160-layer \condense$^\emph{{light}}$ and a 182-layer \condense{} with alternative state-of-the-art CNN architectures.
%Note that we exclude some of the results that achieved by extremely large models or model ensembles, as we are mainly interested in computational efficiency here.
Following \cite{zoph2017learning}, our models were trained for 600 epochs. From the results, we observe that \condense{} requires approximately $8\times$ fewer parameters and FLOPs to achieve a comparable accuracy to DenseNet-190. \condense{} seems to be less parameter-efficient than \condense$^\emph{{light}}$, but is more compute-efficient. Somewhat surprisingly, our \condense$^\emph{{light}}$ model performs on par with the NASNet-A, an architecture that was obtained using an automated search procedure over $20,000$ candidate architectures composed of a rich set of components, and is thus carefully tuned on the CIFAR-10 dataset \cite{zoph2017learning}. Moreover, \condense{} (or \condense$^\emph{{light}}$)
%\lvdm{You mean DenseNet-LGC? In general, I think we should try and come up with a more consistent nomenclature. Right now, \condense is a Fully DenseNet-LGC + increasing growth rate or something like that? This quickly gets very confusing for the reader.}
does not use depth-wise separable convolutions, and only use simple convolutional filters with size $1\!\times\!1$ and $3\!\times\!3$. It may be possible to include \condense{} as a meta-architecture in the procedure of \cite{zoph2017learning} to obtain even more efficient networks.


\begin{table}[]
\addtolength{\tabcolsep}{0pt}
\centering
\small
\resizebox{0.48\textwidth}{!}{
\begin{tabular}{l|rrll}
\hline
\textbf{Model}               					& \textbf{Params}	& \textbf{FLOPs}			& \textbf{C-10}		& \textbf{C-100} \\ \hline
%ResNet-110\cite{resnet}           		& 1.7M		& 254M			& 6.41		& 27.22	\\ \hline
ResNet-1001\cite{identity-mappings}     & 16.1M		& 2,357M		& 4.62		& 22.71	\\
Stochastic-Depth-1202\cite{stochastic}       	& 19.4M		& 2,840M		& 4.91		& -	\\
Wide-ResNet-28\cite{wide}       		& 36.5M    	& 5,248M        & 4.00   	& 19.25     \\
ResNeXt-29 \cite{resnext}          		& 68.1M    	& 10,704M       & 3.58   	& 17.31     \\
%{ShakeShake}\cite{gastaldi2017shake}	& 2.9M 		& 452M			& 3.55		& - 		\\ \hline
%DenseNet-100         & 0.8M     & 297M                  & 4.51   		& 22.27     \\ \hline
DenseNet-190\cite{huang2017densely}		& 25.6M    	& 9,388M		& 3.46  	& 17.18     \\
NASNet-A$^*$\cite{zoph2017learning}		& 3.3M     	& -             & 3.41    	& -         \\ \hline
%NASNet-A$^*$\cite{zoph2017learning}		& 2.6M     	& -             & 3.73    	& -         \\ \hline
%NASNet-A$^*$\cite{zoph2017learning}		& 3.1M     	& -             & 3.59    	& -         \\ \hline
\condense$^\emph{\text{light}}$-160$^*$     					& 3.1M  	& 1,084M 		& 3.46		& 17.55	\\
\condense-182$^*$   				& 4.2M     	& 513M	        & 3.76 		& 18.47     \\
\hline
\end{tabular}
}
\vspace{2pt}
\caption{Comparison of classification error rate (\%) with other convolutional networks on the CIFAR-10(C-10) and CIFAR-100(C-100) datasets. * indicates models that are trained with cosine shape learning rate for 600 epochs.}
\label{tab:cifar}
\end{table}


\paragraph{Comparison with existing pruning techniques.}
In Table~\ref{tab:compare-prune}, we compare our \condense{}s and \condense s$^\emph{{light}}$ with models that are obtained by state-of-the-art \emph{filter-level} weight pruning techniques \cite{li2016pruning,liu2017learning,he2017channel}. The results show that, in general, \condense{} is about $3\times$ more efficient in terms of FLOPs than ResNets or DenseNets pruned by the method introduced in \cite{liu2017learning}. The advantage over the other pruning techniques is even more pronounced. We also report the results for \condense$^\emph{{light}}$ in the second last row of Table~\ref{tab:compare-prune}. It uses only half the number of parameters to achieve comparable performance as the most competitive baseline, the 40-layer DenseNet described by \cite{liu2017learning}.



\begin{table}[]
\addtolength{\tabcolsep}{0pt}
\centering
\small
\resizebox{0.48\textwidth}{!}{
\begin{tabular}{l|rrrr}
\hline
\textbf{Model}  & \textbf{FLOPs} & \textbf{Params} & \textbf{C-10} & \textbf{C-100} \\
\hline
%VGG-16 						& $3.13\times 10^8$ 	&  $15M$  		&   6.75  \\
VGG-16-pruned \cite{li2016pruning} 				& 206M 	&  5.40M   	&   6.60	& 25.28 \\
VGG-19-pruned \cite{liu2017learning} 			& 195M 	&  2.30M   	&   6.20 	&  - \\
VGG-19-pruned \cite{liu2017learning} 			& 250M 	&  5.00M   	&   -	 	& 26.52 \\
\hline
ResNet-56-pruned \cite{he2017channel}			& 62M	&  		&   8.20	& - \\
ResNet-56-pruned \cite{li2016pruning}			& 90M 	&  0.73M	&	6.94	& - \\
%VGG-16-pruned scratch 		&  &  & 6.88 \\
%ResNet-110					& $2.53\times 10^8$ 	&  $1.72\times 10^6$  	&   6.47  \\
ResNet-110-pruned \cite{li2016pruning}			& 213M 	&  1.68M   	&   6.45 	& - \\
%ResNet-110-pruned scratch 	&  &  & 6.88 \\
%ResNet-164-BC				& $5.33\times 10^8$ 	&  $1.70\times 10^6$  	&   5.42  \\
%ResNet-164-B-pruned \cite{liu2017learning}	& 166M 	&  1.45M  	&   5.08		& 22.87  \\
ResNet-164-B-pruned \cite{liu2017learning}	& 124M 	&  1.21M  	&   5.27		& {23.91}  \\
\hline
%DenseNet-40					& $5.33\times 10^8$ 	&  $1.02\times 10^6$  	&   6.11  \\
DenseNet-40-pruned \cite{liu2017learning}	& 190M 	&  0.66M   	&   5.19		& 25.28 \\
\hline
\condense$^\emph{\text{light}}$-94							& 122M 	&  0.33M  	&   {5.00} & 24.08 \\
\condense-86						& 65M 	&  0.52M  	&   {5.00} & {23.64} \\
\hline
\end{tabular}
}
\vspace{2.0pt}
\caption{Comparison of classification error rate (\%) on CIFAR-10 (C-10) and CIFAR-100 (C-100) with state-of-the-art filter-level weight pruning methods.}
\vspace{-1ex}
\label{tab:compare-prune}
\end{table}







%\renewcommand{\arraystretch}{1.1}
\renewcommand{\arraystretch}{1.0}
\begin{table}[!t]
\addtolength{\tabcolsep}{5pt}
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\centering
%\scriptsize
\small
%\resizebox{0.45\textwidth}{!}{%
{
%\begin{tabular}{c|c|c}
%\hline
%\multirow{2}{*}{Output Size} & \condense-74($k\!=\!8$)          & \condense-74($k\!=\!8$)        \\ \cline{2-3}
%                             & \group{8}{8}{8}{|}    & \group{4}{4}{4}{}    \\ \hline
%\cross{112}                  & \multicolumn{2}{c}{\cross{3} conv, stride 2} \\ \hline
%\cross{112}                  & \conv{4}{8}{8}        & \conv{4}{8}{4}       \\ \hline
%\cross{56}                   & \multicolumn{2}{c}{\cross{2} average pool, stride 2}\\ \hline
%\cross{56}                   & \conv{6}{8}{8}        & \conv{6}{8}{4}       \\ \hline
%\cross{28}                   & \multicolumn{2}{c}{\cross{2} average pool, stride 2}\\ \hline
%\cross{28}                   & \conv{8}{8}{8}        & \conv{8}{8}{4}       \\ \hline
%\cross{14}                   & \multicolumn{2}{c}{\cross{2} average pool, stride 2}\\ \hline
%\cross{14}                   & \conv{10}{8}{8}       & \conv{10}{8}{4}       \\ \hline
%\cross{7}                    & \multicolumn{2}{c}{\cross{2} average pool, stride 2}\\ \hline
%\cross{7}                    & \conv{8}{8}{8}        & \conv{8}{8}{4}       \\ \hline
%\cross{1}                    & \multicolumn{2}{c}{\cross{7} global average pool}\\ \cline{1-3}
%                             & \multicolumn{2}{c}{1000-dim fully-connected, softmax}\\ \hline
%\multicolumn{1}{c|}{FLOPs}   & 274M                &   529M               \\ \hline
%\end{tabular}

\begin{tabular}{c|c}
\hline
\textbf{\condense}       	& \textbf{Feature map size}				   \\ \hline
\cross{3} Conv (stride $2$) 			& \cross{112}                  \\ \hline
\conv{4}{8}	        				& \cross{112}                  \\ \hline
\cross{2} average pool, stride 2 	& \cross{56}                   \\ \hline
\conv{6}{16}        				& \cross{56}                   \\ \hline
\cross{2} average pool, stride 2 	& \cross{28}                   \\ \hline
\conv{8}{32}        				& \cross{28}                   \\ \hline
\cross{2} average pool, stride 2 	& \cross{14}                   \\ \hline
\conv{10}{64}       				& \cross{14}                   \\ \hline
\cross{2} average pool, stride 2 	& \cross{7}                    \\ \hline
\conv{8}{128}        				& \cross{7}                    \\ \hline
\cross{7} global average pool 		& \cross{1}                    \\ \hline
1000-dim fully-connected, softmax 	&   						   \\ \hline
\end{tabular}
}
\vspace{1 ex}
\caption{\condense{} architectures for ImageNet.}
%\caption{DenseNet architectures for ImageNet. The growth rate for the first 3 networks is $k=32$, and $k=48$ for DenseNet-161. Note that each ``conv'' layer shown in the table corresponds the sequence BN-ReLU-Conv.   }
\label{tab:structure-imagenet}
\vspace{-3 ex}
\end{table}







\subsection{Results on ImageNet}
\vspace{-1ex}
In a second set of experiments, we test \condense{} on the ImageNet dataset.

\paragraph{Model configurations.}
Detailed network configurations are shown in Table~\ref{tab:structure-imagenet}. To reduce the number of parameters, we prune 50\% of weights from the fully connected (FC) layer at epoch 60 in a way similar to the \methodname{}, but with $G\!=\!1$ (as the FC layer could not be split into multiple groups) and $C\!=\!2$. Similar to prior studies on MobileNets and ShuffleNets, we focus on training relatively small models that require less than 600 million FLOPs to perform inference on a single image.

\paragraph{Training details.}
We train all models using stochastic gradient descent (SGD) with a batch size of 256. As before, we adopt Nesterov momentum with a momentum weight of 0.9 without dampening, and a weight decay of $10^{-4}$. All models are trained for 120 epochs, with a cosine shape learning rate which starts from 0.1 and gradually reduces to 0. We use group lasso regularization in all experiments on ImageNet; the regularization parameter is set to $10^{-5}$.

\paragraph{Comparison with state-of-the-art efficient CNNs.}
Table~\ref{tab:imagenet} shows the results of \condense{}s and several state-of-the-art, efficient models on the ImageNet dataset. We observe that a \condense{}  with 274 million FLOPs obtains a 29.0\% Top-1 error, which is comparable to the accuracy achieved by MobileNets and ShuffleNets that require twice as much compute. A \condense{} with 529 million FLOPs produces to a 3\% absolute reduction in top-1 error compared to a MobileNet and a ShuffleNet of comparable size. Our \condense{} even achieves a the same accuracy with slightly fewer FLOPs and parameters than the most competitive NASNet-A, despite the fact that we only trained a very small number of models (as opposed to the study that lead to the NASNet-A model).

\paragraph{Actual inference time.}
Table~\ref{tab:wall-time} shows the actual inference time on an ARM processor for different models. The wall-time to inference an image sized at $224\times 224$ is highly correlated with the number of FLOPs of the model. Compared to the recently proposed MobileNet, our \condense{} ($G\!=\!C\!=\!8$) with 274 million FLOPs inferences an image $2\times$ faster, while without sacrificing accuracy.

%it even uses slightly fewer FLOPs and parameters to achieve comparable performance as the NASNet, which has a complicated architecture obtained via searching from over thousands of candidates. The \condense{} with 294 million FLOPs yields a 28.2\% test error, also outperforming MobileNet and ShuffleNet by a large margin.

%\begin{table*}[!t]
%\centering
%\begin{tabular}{lcccc}
%\hline
%Model     & FLOPs & \#Paras & Top 1 Acc. (\%) & Top 5 Acc. (\%) \\ \hline
%Inception V1       & 1,448 M                     & 6.6M                 & 69.8                     & 89.9                     \\
%1.0 MobileNet-224  & 569 M                       & 4.2M                 & 70.6                     & 89.5                     \\
%ShuffleNet 2x      & 524 M                       & 5M                   & 70.9                     & 89.8                     \\
%NASNet-A (N=4)     & 564 M                       & 5.3M                 & 74.0                     & 91.6                     \\
%\textbf{\todo{}}   & \textbf{542M}               & \textbf{4.7M}        & \textbf{74.1}            & \textbf{91.7}            \\ \hline
%0.75 MobileNet-224 & 325M                        & 2.3M                 & 68.4                     & -                        \\
%ShuffleNet 1.5x    & 292M                        &                      & 69.0                     & -                        \\
%\textbf{\todo{}}   & \textbf{294M}               & \textbf{2.9M}        & \textbf{69.9}            & \textbf{89.4}            \\ \hline
%%0.5 MobileNet-224  & 149M                        & -                    & 63.7                     & -                        \\
%%ShuffleNet 1x      & 140                         & -                    & 65.9                     & -                        \\
%%\todo{}            &                             &                      &                          &                          \\ \bottomrule
%\end{tabular}
%\caption{Accuracy versus computational budget of state-of-the-art network architectures on ImageNet 2012 ILSVRC challenge classification task. Floating-point Multiply-Add number to process a single image is used to measure the computational budget.}
%\label{tab:imagenet}
%\end{table*}


\renewcommand{\arraystretch}{1.1}
\begin{table}[!t]
\centering
\small
%\scriptsize
\addtolength{\tabcolsep}{-3pt}
\begin{tabular}{l|rrrr}
\hline
\textbf{Model}     & \textbf{FLOPs} & \textbf{Params} & \textbf{Top-1} & \textbf{Top-5} \\ \hline
%0.75 MobileNet-224 \cite{howard2017mobilenets} & 325M                        & 2.3M                 & 31.6                     & 11.8                     \\
%ShuffleNet 1.5x \cite{zhang2017shufflenet}    & 292M                        & 3.3M                    & 31.0                     & -                        \\\hline
%flops:    294.494804 M     params:     2978180.0
%\blue\condense	   &  \blue{294M}      &  \blue{3.0M}			        & \blue{\textbf{28.2}}            &\blue{\textbf{9.6}}            \\ \hline
Inception V1 \cite{szegedy2015going}       & 1,448M                     & 6.6M                 & 30.2                     & 10.1                     \\
1.0 MobileNet-224 \cite{howard2017mobilenets}  & 569M                       & 4.2M                 & 29.4                     & 10.5                     \\
ShuffleNet 2x  \cite{zhang2017shufflenet}    & 524M                       & 5.3M                   & 29.1                     & 10.2                     \\
NASNet-A (N=4) \cite{zoph2017learning}    & 564M                       & 5.3M                 & {26.0}   & 8.4                     \\
NASNet-B (N=4) \cite{zoph2017learning}    & 488M                       & 5.3M                 & {27.2}   & 8.7                     \\
NASNet-C (N=3)  \cite{zoph2017learning}   & 558M                       & 4.9M                 &{27.5}   & 9.0                     \\\hline
%flops:    529.327764 M     params:     4773444.0
\condense{} ($G\!=\!C\!=\!8$)	   &  {274M}      &  {2.9M}	        & {{29.0}}            &{{10.0}}  \\
\condense{} ($G\!=\!C\!=\!4$)   & 529M		       & 4.8M	        & 26.2	          & {8.3}            \\ \hline
\end{tabular}
\vspace{2ex}
\caption{Comparison of \emph{Top-1} and \emph{Top-5} classification error rate (\%) with other state-of-the-art compact models on ImageNet.}
\label{tab:imagenet}
\vspace{-2ex}
\end{table}

\renewcommand{\arraystretch}{1.1}
\begin{table}[!t]
\centering
\small
%\scriptsize
\addtolength{\tabcolsep}{-3pt}
\begin{tabular}{l|rrcc}
\hline
\textbf{Model}     										& \textbf{FLOPs} 	& \textbf{Top-1} 	& \textbf{Time(s)}	 	\\ \hline
VGG-16      								    & 15,300M	& 28.5		& 354		\\
ResNet-18       								& 1,818M	& 30.2		& 8.14		\\
1.0 MobileNet-224 \cite{howard2017mobilenets}  	& 569M		& 29.4		& 1.96		\\
\condense{}  ($G\!=\!C\!=\!4$)					& 529M 		& 26.2		& 1.89 		\\
\condense{}  ($G\!=\!C\!=\!8$)					& 274M 		& 29.0		& 0.99 		\\ \hline
\end{tabular}
\vspace{2ex}
\caption{Actual inference time of different models on an ARM processor. All models are trained on ImageNet, and accept input with resolution 224$\times$224.}
\label{tab:wall-time}
\vspace{-2ex}
\end{table}


\begin{figure*}[ht]
	\centering
	\includegraphics[width=0.33 \textwidth]{plots/pruned.pdf}
    \includegraphics[width=0.33 \textwidth]{plots/groups.pdf}
	\includegraphics[width=0.33 \textwidth]{plots/condense_factor.pdf}
	\caption{Classification error rate (\%) on CIFAR-10. \emph{Left}: Comparison between our condense method with traditional pruning approach, under varying condensation factors. \emph{Middle}: \condense{}s with different number of groups for the $1\!\times\! 1$ \methodname{}. All the models have the same number of parameters. \emph{Right}: \condense{}s with different condensation factors. }
	\label{fig:vary-G-C}
\vspace{-2 ex}
\end{figure*}


\subsection{Ablation Study}
\vspace{-1ex}
We perform an ablation study on CIFAR-10 in which we investigate the effect of (1) the pruning strategy, (2) the number of groups, and (3) the condensation factor. We also investigate the stability of our weight pruning procedure.

\paragraph{Pruning strategy.}
The left panel of \figurename~\ref{fig:vary-G-C} compares our \emph{on-the-fly} pruning method with the more common approach of pruning weights of \emph{fully converged} models. We use a DenseNet with $50$ layers as the basis for this experiment. We implement a ``traditional'' pruning method in which the weights are pruned in the same way as in as in \condense{}s, but the pruning is only done once after training has completed (for 300 epochs). Following~\cite{liu2017learning}, we fine-tune the resulting sparsely connected network for another 300 epochs with the same cosine shape learning rate that we use for training \condense{}s. We compare the traditional pruning approach with the \condense{} approach, setting the number of groups $G$ is set to $4$. In both settings, we vary the condensation factor $C$ between $2$ and $8$.

The results in \figurename~\ref{fig:vary-G-C} show that pruning weights gradually during training outperforms pruning weights on fully trained models. Moreover, gradual weight pruning reduces the training time: the ``traditional pruning'' models were trained for $600$ epochs, whereas the \condense{}s were trained for $300$ epochs. The results also show that removing 50\% the weights (by setting $C\!=\!2$) from the $1 \!\times\! 1$ convolutional layers in a DenseNet incurs hardly any loss in accuracy.



\paragraph{Number of groups.} In the middle panel of \figurename~\ref{fig:vary-G-C}, we compare four \condense{}s with exactly the same network architecture, but a number of groups, $G$, that varies between $1$ and $8$. We fix the condensation factor, $C$, to 8 for all the models, which implies all models have the same number of parameters after training has completed. In \condense{}s with a single group, we discard entire filters in the same way that is common in filter-pruning techniques \cite{li2016pruning,liu2017learning}. The results presented in the figure demonstrate that test errors tends to decrease as the number of groups increases. This result is in line with our analysis in Section \ref{sec:method}, in particular, it suggests that grouping filters gives the training algorithm more flexibility to remove redundant weights.

%\begin{figure}[ht]
%	\centering
%	\includegraphics[width=0.40 \textwidth]{plots/condense_factor.pdf}
%	\caption{CondensedNets with different condense factors on CIFAR-10.}
%	\label{fig:condense-factor}
%\end{figure}

\begin{figure}[t]
	\centering
	\includegraphics[width=0.48 \textwidth]{plots/learned_weights_stablity.pdf}
	\caption{Norm of weights between layers of a CIFAR-10 \condense{} per filter group (\emph{top}) and per filter block (\emph{bottom}). The three columns correspond to independent training runs.}
	\label{fig:learned-weights-stablity}
\vspace{-2ex}
\end{figure}

\paragraph{Effect of the condensation factor.} In the right panel of \figurename~\ref{fig:vary-G-C}, we compare \condense{}s with varying condensation factors. Specifically, we set the condensation factor $C$ to 1, 2, 4, or 8; this corresponds to removing 0\%, 50\%, 75\%, or 87.5\% of the weights from each of the $1\!\times\! 1$ convolutional layers, respectively. A condensation factor $C\!=\!1$ corresponds to a baseline model without weight pruning. The number of groups, $G$, is set to 4 for all the networks.
The results show that a condensation factors $C$ larger than 1 consistently lead to improved efficiency, which underlines the effectiveness of our method. Interestingly, models with condensation factors 2, 4 and 8 perform comparably in terms of classification error as a function of FLOPs. This suggests that whilst pruning more weights yields smaller models, it also leads to a proportional loss in accuracy.


%\begin{figure}[ht]
%	\centering
%	\includegraphics[width=0.40 \textwidth]{plots/pruned.pdf}
%	\caption{Comparison between our model condense method with traditional pruning method, under different condense factors.}
%	\label{fig:traditional-prune}
%\end{figure}






%
%\subsection{Ablation study}
%CondensedNet-$\delta$ (remove dense connection between dense block)
%
%CondensedNet-dw (remove depthwise separable connection)
%
%CondensedNet-group (remove grouped convolution)

%
%\begin{figure}[ht]
%	\centering
%	\includegraphics[height=3.0in]{plots/learned_weights.pdf}
%	\caption{Visualization of weights for CondensedNet-Lite on ImageNet.}
%	\label{fig:learnedWeights}
%\end{figure}



\paragraph{Stability.} As our method removes redundant weights in early stages of the training process, a natural question is whether this will introduce extra variance into the training. Does early pruning remove some of the weights simply because they were initialized with small values?

To investigate this question, \figurename~\ref{fig:learned-weights-stablity} visualizes the learned weights and connections for three independently trained \condense{}s on CIFAR-10 (using different random seeds). The top row shows detailed weight strengths (averaged absolute value of non-pruned weights) between a filter group of a certain layer (corresponding to a column in the figure) and an input feature map (corresponding to a row in the figure). For each layer there are four filter groups (consecutive columns). A white pixel in the top-right corner indicates that a particular input feature was pruned by that layer and group.
Following \cite{huang2017densely}, the bottom row of \figurename~{fig:learned-weights-stablity} shows the overall connection strength between two layers in the condensed network. The vertical bars correspond to the linear classification layer on top of the \condense{}. The gray vertical dotted lines correspond to pooling layers that decrease the feature resolution.

The results in the figure suggest that while there are differences in learned connectivity at the filter-group level (top row), the overall information flow between layers (bottom row) is similar for all three models. This suggests that the three training runs learn similar global connectivity patterns, despite starting from different random initializations. Later layers tend to prefer more recently generated features, do however utilize some features from very early layers.
%The results also seem to suggest that for a given dataset and a given DenseNet architecture, there exists an ``intrinsic connection spectrum'' that our training procedure discovers.


==> arXiv 20180607/intro.tex <==
%!TEX root = main.tex
\vspace{-2ex}
\section{Introduction}
%\vspace{-1ex}
The high accuracy of convolutional networks (CNNs) in visual recognition tasks, such as image classification \cite{vgg,resnet,huang2017densely}, has fueled the desire to deploy these networks on platforms with limited computational resources, \emph{e.g.}, in robotics, self-driving cars, and on mobile devices. Unfortunately, the most accurate deep CNNs, such as the winners of the ImageNet \cite{deng2009imagenet} and COCO \cite{lin2014microsoft} challenges, were designed for scenarios in which computational resources are abundant. As a result, these models cannot be used to perform real-time inference on low-compute devices.

This problem has fueled development of computationally efficient CNNs that, \emph{e.g.}, prune redundant connections \cite{lecun1989optimal,hassibi1993optimal,li2016pruning,liu2017learning,han2015deep}, use low-precision or quantized weights \cite{hubara2016binarized,rastegari2016xnor,chen2015compressing}, or use more efficient network architectures \cite{iandola2016squeezenet,resnet,huang2017densely,chollet2016xception,howard2017mobilenets,zhang2017shufflenet}. These efforts have lead to substantial improvements: to achieve comparable accuracy as VGG~\cite{vgg} on ImageNet, ResNets \cite{resnet} reduce the amount of computation by a factor $5 \times$, DenseNets \cite{huang2017densely} by a factor of $10 \times$, and MobileNets \cite{howard2017mobilenets} and ShuffleNets \cite{zhang2017shufflenet} by a factor of $25\times$. A typical set-up for deep learning on mobile devices is one where CNNs are trained on multi-GPU machines but deployed on devices with limited compute. Therefore, a good network architecture allows for fast parallelization during training, but is compact at test-time.


%Among them, innovations on network architectures are arguably the most fundamental and fruitful for developing more efficient deep models. For example, the residual network (ResNet) architecture \cite{resnet} uses 5 times fewer computation to achieve the same accuracy as the VGG network \cite{vgg} on the ImageNet classification dataset, while the DenseNet architecture \cite{huang2017densely} further cuts the computation by half compared to ResNet. The most recent developments along this direction adopt a variant of convolution operation, named depthwise separable convolution \cite{chollet2016xception}, to build computationally efficient CNNs \cite{howard2017mobilenets,zhang2017shufflenet}. By leveraging depthwise separable convolution, the MobileNets and ShuffleNets achieve VGG-level accuracy on ImageNet but using only 1/25 the amount of computation as the VGG network.



Recent work~\cite{chen2015compressing,stochastic} shows that there is a lot of redundancy in CNNs. The layer-by-layer connectivity pattern forces networks to replicate features from earlier layers throughout the network. The DenseNet architecture \cite{huang2017densely} alleviates the need for feature replication by directly connecting each layer with all layers before it, which induces feature re-use.
%The goal of this paper is to explore whether further reductions in compute can be achieved whilst maintaining VGG-level accuracies on ImageNet.
Although more efficient, we hypothesize that dense connectivity introduces redundancies when early features are not needed in later layers. We propose a novel method to prune such redundant connections between layers and then introduce a more efficient architecture. In contrast to prior pruning methods, our approach learns a sparsified network automatically during the training process, and  produces a regular connectivity pattern that can be implemented efficiently using group convolutions. Specifically, we split the filters of a layer into multiple groups, and gradually remove the connections to less important features \emph{per group} during training. Importantly, the groups of incoming features are not predefined, but \emph{learned}. The resulting model, named \condense,  can be trained efficiently on GPUs, and has high inference speed on mobile devices.

%On one hand, dense connectivity reduces parameter/computational redundancy by allowing deep layers to reuse features computed from earlier layers. On the other hand, it also introduces redundant connections if these features are not necessary in later layers. This raises a question that if we can design a more compact network with less dense connections, such that each layer can selectively depend on a subset of most important inputs?

%To this end,  we introduce a simple but effective approach to learn highly efficient convolutional networks, particularly under the setting that the models are \emph{trained} on GPUs, and \emph{deployed} on mobile devices or other applications with limited computational resource. Our motivation is to simplify the DenseNet architecture by sparsifying its connections across layers, meanwhile with the following goals achieved simultaneously: (1) the sparsified network is highly regular and only requires dense matrix operation, which is efficiently implemented by existing deep learning libraries; (2) it is able to reduce the computational complexity to a pre-specified budget exactly; (3) minimal overhead is added to the training process compared to training a normal DenseNet.

%We achieve this goal by first splitting the filters of a convolutional layer into multiple groups, and at the early stage of training we gradually remove the connections to those less important features \emph{for each group}. Thus a large portion of redundant connections will be pruned, yielding significantly more compact models. Different from most pruning techniques, our algorithm has the nice property that the convolutional layers with pruned weights can then be cast as standard \emph{group convolution}, a well supported operation by most deep learning libraries. Since the \emph{input} feature groups are formed during the learning process, we call this layer \emph{\methodname}, to differential from traditional group convolution with predefined groups. It is noteworthy \methodname{} is also more flexible, as different filter groups may simultaneously use a same feature, and some features may not be used by any group.

%To this end, we propose a specially designed algorithm to enhance the feature reuse in DenseNet. It is a simple approach that can automatically screen out less useful incoming features for a given layer and leaving the most important features for reuse. Compared to most existing weight pruning techniques, our algorithm has two prominent advantages: (1) the sparsified models still enjoy the benefit of highly efficient dense matrix operations; (2) it adds little computation overhead to the training process as it does not require a long pipeline of fine-tuning after pre-training and pruning.


Our image-classification experiments show that \condense{}s consistently outperform alternative network architectures. Compared to DenseNets, \condense{}s use only $1/10$ of the computation at comparable accuracy levels. On the ImageNet dataset \cite{deng2009imagenet}, a \condense{} with 275 million FLOPs\footnote{Throughout the paper, \emph{FLOPs} refers to the number of multiplication-addition operations.} achieved a 29\% top-1 error, which is comparable to the error of a MobileNet that requires twice as much compute.


%We further introduce an improved DenseNet architecture, \modelname{}, to complement our algorithm. \modelname{} simplifies the original architecture by allowing a direct connection between any two layers in the network, even their output feature map sizes do not match. This enables the network to reuse features more directly and extensively. To ensure the incoming feature maps for a given convolutional layer have the same resolution, we simply down-sample large feature maps by average pooling. Another change is that we always double the \emph{growth rate}, i.e., the number of features produced by a basic DenseNet layer, after each down-sampling operation. This lead to an architecture with a similar spirit as the Pyramid Residual Network \cite{han2016deep}. These two changes together lead to greatly improved computational efficiency.

%The \methodname{} is essentially a convolutional layer with pruned weights. However, the pruning technique we used here achieves a sparsity level between the (2D) kernel level sparsity and the (3D) filter level sparsity \cite{Mao}. Our method is much more flexible than pruning filter as that in \cite{li2016pruning,liu2017learning}, as different groups have the freedom to use different sets of features. Meanwhile, our obtained models have higher regularity than pruning kernels, as it can be casted as standard group convolution which requires no special hardware/software accelerator for fast inference.



==> arXiv 20180607/macros.tex <==
% METHOD NAME

\newcommand{\modelname}{DenseNet-{Lite}}
\newcommand{\methodname}{learned group convolution}
\newcommand{\methodnamecap}{Learned Group Convolution}
\newcommand{\methodnameshort}{LGC}
\newcommand{\condense}{CondenseNet}

\newcommand{\methodblock}{dense block}
\newcommand{\methodblockcap}{Dense Block}

\newcommand{\regmethodname}{feature drop}
\newcommand{\regmethodnamecap}{Feature Drop}

\newcommand{\stepsizename}{growth rate}

\newcommand{\red}[1]{\textcolor{red}{#1}}
\newcommand{\blue}[1]{\textcolor{blue}{#1}}

%\newcommand{\bold}[1]{\textbf{#1}}

\newcommand{\conv}[2]{$
\left[
\begin{array}{ll}
%\text{1}\times \text{1} \text{ L-conv} \\
{1}\!\times\! {1} \text{ L-Conv} \\
%\text{(G=#2, C=#2)} \\
%\text{3}\times \text{3} \text{ G-conv} \\
{3}\!\times\! {3} \text{ G-Conv} \\
%\text{(G=#2)} \\
\end{array}
\right] \!\times\! {#1} \quad (k\!=\!#2)$}

%\newcommand{\group}[4]{\multicolumn{1}{c#4}{$
%\begin{array}{l}
%G = #1\\
%C = #2\\
%G = #3
%\end{array}$}}

\newcommand{\group}[4]{\multicolumn{1}{c#4}{$\text{G = #1, C = #2, G = #3}$}}

\newcommand{\cross}[1]{$#1 \!\times\! #1$}

% Gradients Equations
\newcommand{\feati}{x_i}
%\newcommand{\concatfeati}{x_i}
\newcommand{\clsfeati}{y_i}
\newcommand{\featk}{x_k}
\newcommand{\clsfeatk}{y_k}
\newcommand{\loss}{L}
\newcommand{\featL}{x_L}
\newcommand{\clsfeat}{y}
% Inputs and outputs
\newcommand{\anyxs}{\ensuremath{\mathbf{x}}}
\newcommand{\anyys}{\ensuremath{\mathbf{y}}}

\newcommand{\bF}{\ensuremath{\mathbf{F}}}
\newcommand{\bM}{\ensuremath{\mathbf{M}}}

\newcommand{\bx}{\ensuremath{\mathbf{x}}}

\newcommand{\sourcexs}{\ensuremath{\mathbf{x^\mathcal{S}}}}
\newcommand{\sourceys}{\ensuremath{\mathbf{y^\mathcal{S}}}}

\newcommand{\targetxs}{\ensuremath{\mathbf{x^\mathcal{T}}}}
\newcommand{\targetys}{\ensuremath{\mathbf{y^\mathcal{T}}}}
\newcommand{\pseudotargetys}{\ensuremath{\mathbf{\hat{y}^\mathcal{T}}}}



==> arXiv 20180607/method.tex <==
%!TEX root = main.tex


\section{\condense s}
\label{sec:method}

Group convolution works well with many deep neural network architectures~\cite{resnext,zhang2017shufflenet,zhang2017interleaved} that are connected in a layer-by-layer fashion.
For dense architectures group convolution can be used in the $3\!\times \!3$ convolutional layer (see Figure~\ref{fig:structure_compare}, left). However, preliminary experiments show that a na\"ive adaptation of group convolutions in the $1\!\times \!1$ convolutional layer leads to drastic reductions in accuracy. We surmise that this is caused by the fact that the inputs to the $1\!\times \!1$ convolutional layer are concatenations of feature maps generated by preceding layers. Therefore, they differ in two ways from typical inputs to convolutional layers: 1. they have an intrinsic order; and 2. they are far more diverse.
% DenseNets have an intrinsic order, as they are concatenations of feature maps from prior layers; and 2. dense connectivity is known to reduce the feature redundancy present in layer-by-layer connectivity~\cite{stochastic,huang2017densely}.
%This is consistent with recent evidence~\cite{stochastic} that show that this connectivity pattern induces feature redundancy.
The hard assignment of these features to disjoint groups hinders effective re-use of features in the network.
Experiments in which we randomly permute input feature maps in each layer before performing the group convolution show that this reduces the negative impact on accuracy --- but even with the random permutation, group convolution in the $1\!\times \!1$ convolutional layer makes DenseNets less accurate than for example smaller DenseNets with equivalent computational cost.

%Huang et al.~\cite{huang2017densely} have shown that it is important to make early features available as inputs to later layers. 
It is shown in \cite{huang2017densely} that making early features available as inputs to later layers is important for efficient feature re-use.
Although not all prior features are needed at every subsequent layer, it is hard to predict which features should be utilized at what point.
To address this problem, we develop an approach that \emph{learns} the input feature groupings automatically during training. Learning the group structure allows each filter group to select its own set of most relevant inputs. Further, we allow multiple groups to share input features and also allow features to be ignored by all groups. Note that in a DenseNEt, even if an input feature is ignored by all groups in a specific layer, it can still be utilized by some groups At different layers.
To differentiate it from regular group convolutions, we refer to our approach as \emph{\methodname}.


%This section presents the two key components of \condense{}s: (1) \emph{\methodname{}s} and (2) a fully densely connected network architecture with an exponentially increasing growth rate.

%In this paper, we propose \emph{\methodname}, which forms the feature groups automatically during the training process. In addition, it is more flexible, as it does not need to enforce different groups to use completely disjoint incoming features. It is acceptable that some important features are simultaneously used by multiple groups, while some less important features are never used by that given layer. This is especially desirable for DenseNet, as it allows each layer to decide what features from previous layers should be used.


%In DenseNets, the number of features received by a deep layer is generally quite large, since it corresponds to a concatenation of features from many different layers. To improve the computational efficiency, the original DenseNet uses a convolutional layer with kernel size $1\times 1$ to perform dimension reduction on the incoming features (see the left part of \figurename~\ref{fig:structure_compare}). Even though, it still constitutes a lot of computation.

%Motivated by the grouped convolution, we resort to a structured group sparsity to improve the efficiency of DenseNet-like architectures.
%One explanation why group convolution is not suitable for DenseNets (even with random grouping) is that dense connectivity leads to a substantial reduction in redundancy~\cite{huang2017densely}.
%The success of group convolution shows that it is possible to learn  high quality output features from just a small subset of inputs.  We hypothesize that in the presence of  feature redundancy, restricting feature maps to pre-specified connectivity patterns works well, because it is sufficiently likely that at any given layer some copies of necessary input features  are grouped together in at least some of the groups to create the required output features.

%One of the benefits of dense connectivity is that it allows efficient feature re-use without encouraging redundancy. It is therefore likely that necessary input features are missing and cannot be learned because DenseNets also have far fewer parameters.
%Without loss of generality, we only learn the \emph{input feature groups}, and pre-specify the \emph{output feature groups}; see \figurename~\ref{fig:learned_conv}.

\subsection{\methodnamecap}
\label{subsec:LGC}

We learn group convolutions through a multi-stage process, illustrated in
\figurename{}s~\ref{fig:learned_conv} and \ref{fig:learning-rate}. The first half of the training iterations comprises of \emph{condensing} stages. Here,  we repeatedly train the network with sparsity inducing regularization for a fixed number of iterations and subsequently prune away unimportant filters with low magnitude weights. The second half of the training consists of the \emph{optimization} stage, in which we learn the filters after the groupings are fixed.
When performing the pruning, we ensure that filters from the same group share the same sparsity pattern. As a result, the sparsified layer can be implemented using a standard group convolution once training is completed (\emph{testing} stage). Because group convolutions are efficiently implemented by many deep-learning libraries, this leads to high computational savings both in theory and in practice. We present details on our approach below.
% (starting point of Training Phase I), and then ``condense'' the model by gradually pruning less important connections during training (Training Phase I).

\paragraph{Filter Groups.} We start with a standard convolution of which filter weights form a 4D tensor of size $O\!\times\! R \!\times\! W \!\times\! H$, where $O$, $R$, $W$, and $H$ denote the number of output channels, the number of input channels, and the width and the height of the filter kernels, respectively. As we are focusing on the $1\times 1$ convolutional layer in DenseNets, the 4D tensor reduces to an $O\!\times\! R$ matrix $\bF$. We consider the simplified case in this paper. But our procedure can readily be used with larger convolutional kernels. Before training, we first split the filters (or, equivalently, the output features) into $G$ groups of equal size. We denote the filter weights for these groups by $\bF^1,\ldots,\bF^G$; each $\bF^g$ has size $\frac{O}{G}\!\times\! R$ and $\bF^g_{ij}$ corresponds to the weight of the $j$th input for the $i$th output within group $g$. Because the output features do not have an implicit ordering, this random grouping does not negatively affect the quality of the layer.
%, but it does reduce the number of parameters.

\paragraph{Condensation Criterion.}
During the training process we gradually screen out  subsets of less important input features for each group. The importance of the $j$th incoming feature map for the filter group $g$ is evaluated by the averaged absolute value of weights between them across all outputs within the group, \emph{i.e.}, by $\sum_{i=1}^{{O}/{G}} |\bF^g_{i,j}|$. In other words, we remove columns in $\bF^g$ (by zeroing them out) if their $L_1$-norm is small compared to the $L_1$-norm of other columns. This results in a convolutional layer that is structurally sparse: filters from the same group always receive the same set of features as input.


\paragraph{Group Lasso.} To reduce the negative effects on accuracy introduced by weight pruning,  $L_1$ regularization is commonly used to induce sparsity \cite{li2016pruning,liu2017learning}. In \condense s, we encourage convolutional filters from the same group to use the same subset of incoming features, \emph{i.e.}, we induce group-level sparsity instead. To this end, we use the following group-lasso regularizer \cite{yuan2006model} during training:
\begin{equation}
\label{eq:group-lasso}
\sum\nolimits_{g=1}^G\sum\nolimits_{j=1}^{R}\sqrt{\sum\nolimits_{i=1}^{O/G} {\bF^{g}_{i,j}}^2}. \nonumber
\end{equation}
%Herein, $\bF^{g}_{i,j}$ denotes the element of $\bF^{g}$ at index $(i,j)$.
The group-lasso regularizer simultaneously pushes all the elements of a column of $\bF^g$ to zero, because the term in the square root is dominated by the largest elements in that column. This induces the group-level sparsity we aim for.

\paragraph{Condensation Factor.} In addition to the fact that \methodname{}s are able to automatically discover good connectivity patterns, they are also more flexible than standard group convolutions.
%In \methodname{}, some feature maps may be simultaneously used by multiple groups, while some are not used by any of the groups. This is especially helpful for DenseNet-like architecture to effectively reuse most prominent features and screen out redundant features.
In particular, the proportion of feature maps used by a group does not necessarily need to be $\frac{1}{G}$. We define a \emph{condensation factor} $C$, which may differ from $G$, and allow each group to select $\left\lfloor{\frac{R}{C}}\right\rfloor$ of inputs.

\paragraph{Condensation Procedure.}
In contrast to approaches that prune weights in pre-trained networks, our weight pruning process is integrated into the training procedure. As illustrated in \figurename~\ref{fig:learned_conv} (which uses $C\!=\!3$),
at the end of each  $C\!-\!1$ \emph{condensing} stages we prune $\frac{1}{C}$ of the filter weights.
By the end of training, only $\frac{1}{C}$ of the weights remain in each filter group.  In all our experiments we set the number of training epochs of the condensing stages to $\frac{M}{2(C\!-\!1)}$, where $M$ denotes the total number of training epochs---such that the first half of the training epochs is used for condensing.
%epochs at which a pruning step is performed to , $\frac{2}{2(C\!-\!1)}$, \dots, $\frac{C\!-\!1}{2(C\!-\!1)}$ times the total number of training epoch.
In the second half of the training process, the \emph{Optimization} stage,  we train the sparsified model.\footnote{
In our implementation of the \emph{training} procedure we do not actually remove the pruned weights, but instead mask the filter $\bF$ by a binary tensor $\bM$ of the same size using an element-wise product.
 %$O\!\times\! R \!\times\! W \!\times\! H$.
The mask is initialized with only ones, and elements corresponding to pruned weights are set to zero. This implementation via masking is more efficient on GPUs, as it does not require sparse matrix operations. In practice, the pruning hardly increases the wall time needed to perform a forward-backward pass during training.}

%Surprisingly, training this full model is even faster than training a sparsified model with grouped convolution, thanks to its better parallelization property.

% LAURENS: This is not surprising at all! The implementation of grouped convolutions in cudnn is actually known to be really bad.

\paragraph{Learning rate.} We adopt the \emph{cosine shape learning rate} schedule of Loshchilov et al.~\cite{loshchilov2017sgdr}, which smoothly anneals the learning rate, and usually leads to improved accuracy~\cite{huang2017snapshot,zoph2017learning}. \figurename~\ref{fig:learning-rate} visualizes the learning rate as a function of training epoch (in magenta), and the corresponding training loss (blue curve) of a \condense{} trained on the CIFAR-10 dataset \cite{cifar}. The abrupt increase in the loss at epoch 150 is causes by the final condensation operation, which removes half of the remaining weights. However, the plot shows that the model gradually recovers from this pruning step in the optimization stage.


\paragraph{Index Layer.} After training we remove the pruned weights and convert the sparsified model into a network with a regular connectivity pattern that can be efficiently deployed on devices with limited computational power. For this reason we introduce an \emph{index layer} that implements the feature selection and rearrangement operation (see
\figurename~\ref{fig:learned_conv}, right).
The convolutional filters in the output of the index layer are rearranged
to be amenable to existing (and highly optimized) implementations of regular group convolution. Figure~\ref{fig:structure_compare} shows the transformations of the \condense{} layers during training (middle) and during testing (right). During training the $1\times 1$ convolution is a learned group convolution (L-Conv), but during testing, with the help of the \emph{index} layer, it becomes a standard group convolution (G-Conv).




\begin{figure}[t]
	\centering
	\includegraphics[width=0.5 \textwidth]{plots/learning_curve2.pdf}
	\caption{The cosine shape learning rate and a typical training loss curve with a condensation factor of $C \!=\! 4$.}
	\label{fig:learning-rate}
    \vspace{-2ex}
\end{figure}


\begin{figure}
  % Requires \usepackage{graphicx}
  \centering
  \includegraphics[width=0.5 \textwidth]{plots/full_dense.pdf}\\
  \caption{The proposed DenseNet variant. It differs from the original DenseNet in two ways: (1) layers with different resolution feature maps are also directly connected; (2) the growth rate doubles whenever the feature map size shrinks (far more features are generated in the third, yellow, dense block than in the first).}\label{fig:fully_densenet}
\vspace{-2ex}
\end{figure}



%Although this approach starts with a much larger model compared to a
%Interestingly, although the full model has much larger size compared to the resulting model, it can be trained faster than the latter on GPU, thanks to its better parallelization property. In other words, our method not only yields higher accuracy than standard grouped convolution, but also trains faster.



\subsection{Architecture Design}
\vspace{-1ex}
In addition to the use of \methodname{}s introduced above, we make two changes to the regular DenseNet architecture. These changes are designed to further simplify the architecture and improve its computational efficiency. \figurename~\ref{fig:fully_densenet} illustrates the two changes that we made to the DenseNet architecture.

%\paragraph{Exponentially increasing growth rate.}
\paragraph{Exponentially increasing growth rate.}
The original DenseNet design adds $k$ new feature maps at each layer, where $k$ is a constant referred to as the \emph{growth rate}. As shown in \cite{huang2017densely}, deeper layers in a DenseNet tend to rely on high-level features more than on low-level features. This motivates us to improve the network by strengthening \emph{short-range} connections.
We found that this can be achieved by gradually increasing the growth rate as the depth grows. This increases the proportion of features coming from later layers relative to those from earlier layers. For simplicity, we set the growth rate to $k \!=\! 2^{m-1}k_0$, where $m$ is the index of the dense block, and $k_0$ is a constant. This way of setting the growth rate does not introduce any additional hyper-parameters. The ``increasing growth rate'' (IGR) strategy places a larger proportion of parameters in the later layers of the model. This increases the computational efficiency substantially but may decrease the parameter efficiency in some cases.
Depending on the specific hardware limitations it may be advantageous to trade-off one for the other~\cite{iandola2016squeezenet}.


%\paragraph{Fully dense connectivity.}
\paragraph{Fully dense connectivity.}
To encourage feature re-use even more than the original DenseNet architecture does already, we connect input layers to \emph{all} subsequent layers in the network, even if these layers are located in different dense blocks (see \figurename~\ref{fig:fully_densenet}). As dense blocks have different feature resolutions, we  downsample feature maps with higher resolutions when we use them as inputs into lower-resolution layers using average pooling.


%The original DenseNet uses an uniform growth rate through the whole network, i.e., all layers have the same width. Such design is more parameter efficiency oriented instead of computational efficiency oriented. Compared to the VGG network and ResNet architecture in which the layer width doubles after each down-sampling layer, DenseNets allocate more computation on high resolution feature maps. This tends to improve parameter efficiency, but not computational efficiency. Under the setting where computational efficiency is the major concern, we find it is helpful to double the growth rate after each transition layer in DenseNet.

%\paragraph{Transition Layers} in a DenseNet have much larger width than normal layers in the network. Therefore, they introduce a considerable amount of parameters and computation, although their number is usually small. To address this problem, the original DenseNet architecture uses convolution with filter size $1\times 1$ followed by a pooling layer to construct the transition layer. Even though, the transition layers still account for ~40\% of the full network's computation. We find that simply flip the position of the convolutional layer and the pooling layer, i.e., performing pooling before convolution, leads to a computation reduction of 75\% in transition layers, while causes minimal accuracy loss.


%The new network is complementary to the \methodname{} we introduce above.

%
%\subsection{Discussions}
%We briefly discuss the connections of the proposed method with some existing approaches.
%
%\paragraph{Connection with grouped convolution.}
%Unlike standard grouped convolution, our approach does not need to enforce different groups to use completely disjoint incoming features. It is acceptable that some important features are simultaneously used by multiple groups, while some less important features are never used by that given layer. At test time, we only need to insert an index layer before the grouped convolution to prepare the correct input. This renders more flexibility to the network compared to standard grouped convolution. This is especially desirable for DenseNet, as it allows each layer to decide what features from previous layers should be used.
%
%Interestingly, although the full model has much larger size compared to the resulting model, it can be trained faster than the latter on GPU, thanks to its better parallelization property. In other words, our method not only yields higher accuracy than standard grouped convolution, but also trains faster.
%
%\paragraph{Connection with weight pruning.}
%There are many existing techniques that can be used for learning a sparse model. Most of them adopt the pipeline of using $L1$ regularization during training, followed by pruning and fine tuning. The weight pruning process proposed here is much simpler, as it requires no pre-training or fine tuning. There is no significant overhead added to the training process. In addition, we explore a new level of sparsity that nicely tradeoff between flexibility and regularity. Such sparsity is much more flexible than the filter-level sparsity as long as the number of groups is larger than one; while it only relies on standard grouped convolution, which is well supported by most exist deep learning libraries.


==> arXiv 20180607/related.tex <==
%!TEX root = main.tex

\vspace{-1ex}
\section{Related Work and Background}
\vspace{-1ex}

%\textbf{Network Design.} MobileNet, SqueezedNet, MSDNet, CNNPack, ENet ...
%
%\textbf{Network compression.} Deep compression, prune, hashing, quantization...
%
%The depthwise separable convolution applies large filters, e.g., of size $3 \!\times\! 3$, to each incoming feature map independently, while use the cheaper convolution with filter size $1\!\times \!1$ to combine the resulting feature maps afterwards.


We first review related work on model compression and efficient network architectures, which inspire our work. Next, we review the DenseNets and group convolutions that form the basis for \condense.

\vspace{-1ex}
\subsection{Related Work}
\vspace{-1ex}
%\vspace{-2ex}
\noindent \textbf{Weights pruning and quantization.}
\condense{}s are closely related to approaches that improve the inference efficiency of (convolutional) networks via weight pruning~\cite{lecun1989optimal,hassibi1993optimal,li2016pruning,liu2017learning,he2017channel} and/or weight quantization~\cite{hubara2016binarized,rastegari2016xnor}. These approaches are effective because deep networks often have a substantial number of redundant weights that can be pruned or quantized without sacrificing (and sometimes even improving) accuracy. For convolutional networks, different pruning techniques may lead to different levels of granularity~\cite{Mao}. Fine-grained pruning, \emph{e.g.}, independent weight pruning \cite{lecun1989optimal,han2015learning}, generally achieves a high degree of sparsity. However, it requires storing a large number of indices, and relies on special hardware/software accelerators. In contrast, coarse-grained pruning methods such as filter-level pruning \cite{li2016pruning,alvarez2016learning,liu2017learning,he2017channel} achieve a lower degree of sparsity, but the resulting networks are much more regular, which facilitates efficient implementations.

\condense{}s also rely on a pruning technique, but differ from prior approaches in two main ways: First, the weight pruning is initiated in the early stages of training, which is substantially more effective and efficient than using $L_1$ regularization throughout. Second, \condense{}s have a higher degree of sparsity than filter-level pruning, yet generate highly efficient group convolution---reaching a sweet spot between sparsity and regularity.



%In terms of connection pruning, we  introduce a simple approach to gradually remove less important connections at an early stage of the training process. This algorithm is much more efficient than the traditional weight pruning techniques \cite{lecun1989optimal,hassibi1993optimal,han2015learning,li2016pruning,liu2017learning}, as it does not require the pre-train, pruning and fine-tuning pipeline. Interestingly, our results show that pruning connections on-the-fly is also more \emph{accurate} than pruning a well converged models followed by fine-tuning, possibly due to that the network in an early stage of training  is easier to recover from the ``damage'' caused by pruning.
%

%\vspace{-2ex}
\noindent \textbf{Efficient network architectures.} A range of recent studies has explored efficient convolutional networks that can be trained end-to-end  \cite{huang2017densely,zhang2017interleaved,howard2017mobilenets,zhang2017shufflenet,zoph2017learning,iandola2016squeezenet,zhaodeep}.
%The DenseNet architecture \cite{huang2017densely} allows effective feature reusing in the network, and it requires about 10 times fewer computation than the VGG network to achieve a comparable performance on ImageNet.
Three prominent examples of networks that are sufficiently efficient to be deployed on mobile devices are MobileNet \cite{howard2017mobilenets}, ShuffleNet \cite{zhang2017shufflenet}, and Neural Architecture Search (NAS) networks \cite{zoph2017learning}. All these networks use depth-wise separable convolutions, which greatly reduce computational requirements without significantly reducing accuracy. A practical downside of these networks is depth-wise separable convolutions are not (yet) efficiently implemented in most deep-learning platforms. By contrast, \condense{} uses the well-supported group convolution operation~\cite{alexnet}, leading to better computational efficiency in practice.


\noindent \textbf{Architecture-agnostic efficient inference}
%In addition to studies that develop efficient CNN architectures,
has also been explored by several  prior studies. For example, knowledge distillation \cite{bucilu2006model,hinton2015distilling} trains small ``student'' networks to reproduce the output of large ``teacher'' networks to reduce test-time costs. Dynamic inference methods \cite{bolukbasi2017adaptive,graves2016adaptive,figurnov2016spatially,huang2018multi} adapt the inference to each specific test example, skipping units or even entire layers to reduce computation. We do not explore such approaches here, but believe they can be used in conjunction with \condense{}s.
%Further, adaptive inference methods that selectively evaluate classifiers with increasing cost are proposed in \cite{huang2017multi} and \cite{bolukbasi2017adaptive}.


\begin{figure}
  % Requires \usepackage{graphicx}
  \centering
  \includegraphics[width=0.38 \textwidth]{plots/structure_compare.pdf}\\
  \caption{The transformations within a \emph{layer} in DenseNets \emph{(left)}, and   \condense{}s at training time \emph{(middle)} and at test time \emph{(right)}.  The \emph{Index} and \emph{Permute} operations are explained in Section~\ref{subsec:LGC} and \ref{subsec:cifar}, respectively. (L-Conv: learned group convolution; G-Conv: group convolution) }
  \vspace{-2ex}
  \label{fig:structure_compare}
\end{figure}


\begin{figure}
  % Requires \usepackage{graphicx}
  \centering
  \includegraphics[width=0.45 \textwidth]{plots/group_full_conv.pdf}\\
  \caption{Standard convolution \emph{(left)} and group convolution \emph{(right)}. The latter enforces a sparsity pattern by partitioning the inputs (and outputs) into disjoint groups.  }
  \vspace{-2ex}
  \label{fig:group-conv}
\end{figure}






